Heavy quarks and jets as probes of the QGP

Quark-Gluon Plasma (QGP), a QCD state of matter created in ultra-relativistic heavy-ion collisions, has remarkable properties, including, for example, a low shear viscosity over entropy ratio. By detecting the collection of low-momentum particles that arise from the collision, it is possible to gain quantitative insight into the created matter. However, its fast evolution and thermalization properties remain elusive. Only using high momentum objects as probes of QGP can unveil its constituents at different wavelengths. In this review, we attempt to provide a comprehensive picture of what was, so far, possible to infer about QGP given our current theoretical understanding of jets, heavy-flavor, and quarkonia. We will bridge the resulting qualitative picture to the experimental observations done at the LHC and RHIC. We will focus on the phenomenological description of experimental observations, provide a brief analytical summary of the description of hard probes, and an outlook on the main difficulties we will need to surpass in the following years. To benchmark QGP-related effects, we will also address nuclear modifications to the initial state and hadronization effects.

==> QGPdensity.tex <==

\section{Density of the QGP}


\subsection{Stopping power, viscosity and heavy quark diffusion}
\item Density of the QGP / Properties of the QGP 

    - What are the theoretical connection between QGP density, qhat, eta/s, Debye screen length, temperature and diffusion coefficients?
       - Are they independent info? Are the cross-checks to each other? 
       - How are they related to each other with in a set of underlying assumption?
       - They are evolving as a function of time. What do we mean by "measure" (or "extract") them?
       \textcolor{red}{mw: good!}
       
    - QGP density and qhat from high pt objects (jets, particles)
       - A short reminder of Density of the QGP from particle dN/deta, <pT> and dEt/deta. What are the underlying assumptions? 
          - I realized that we will need to let the reader know when was the QGP produced.
          \textcolor{red}{MW: yes in some way, I think that it is also important to make the point that we put ourselves usually in a context, where viscous corrections are only important very early and where things are quite isentropic later }
       - Why is QGP density and qhat important?
       \textcolor{red}{MW: maybe this is a good point to make a connection in some way to the introduction}
       - Is the color density extracted by jets and particles consistent with the soft probe results?
       - What is the current status of the qhat extraction (largely based on particles only(!))?
          - Extraction from charged particle RAA
          - Extraction from angular correlation of charged particles? 
          - Why do we still have a sizable uncertainty? (Underlying mechanism). 
          - Why is the extraction of qhat from particles not enough and can't we just work on particles?
          - What would be the qhat extracted from jets and jet substructre based observables? Are they consistent with the extracted values from charged particles?
             - What can we say about qhat from jet RAA?
             - What is the expectation on the modification of dijet or photon-jet angular correlation?
             - qhat extraction from Zg
      - Suppose we know very well the qhat, what do we learn?

    - eta/s from quarkonia (changes the lifetime of the medium)
       - Short reminder / reference of the eta/s extraction from flow
       - Different eta/s changes the way QGP evolve (lifetime, density evolution etc) in hydro model. Leads to different suppression pattern of quarkonia
       - Do we see a consistent picture between quarkonia and flow?

    - Temperature of the QGP
       - short reminder of thermal photon extraction
       - Quarkonia are sensitive to temperature. What do we know about the temperature of QGP and consistency between different measurements
       \textcolor{red}{MW: I think that this will be a quite delicate discussion, my idea would be to rather invert it, to say, that the system is such complicated, that we rather invert it: we take the temperature from soft/bulk and we see what happens with quarkonium.... I think that this has to be discussed among us}
       
    - diffusion coefficient from heavy-quarks (also connect to eta/s in some way.)
       - Why is diffusion coefficient important?
       - Lattice predictions, pQCD based predictions for charm and beauty quark diffusion
       - Extraction from D meson v2 and RAA. Why can't we claim victory already?
       - Why do we want to study beauty quarks? (heavier) 
       - Can we relate Ds and eta/s? Do we see an overall consistent picture or not?
       - Why is it important to further improve the diffusion coefficient measurement with future data?
    
\subsection{Thermalization and medium response}
    - What is the motivation to study the thermalization of hard probes?

    
       - To understand how the QGP is produced from many soft scatterings 
       - With hard probes: we look at the thermalization process
       - Can we say more beyond the statement above? for instance, what can we learn about the initial stages of the QGP if we learned how the (semi-)hard probes thermalize?
          - connection to kinetic theory and hydrodynamization
       
    - Thermalization:
        - What is thermalized first? (Soft component)
        - What is never thermalized? (hard part of the jet)
        - What is the connection to charm (or beauty) thermalization? 
        \textcolor{red}{MW: very good!}

    - Medium response/recoil (long wave-length behaviour)
        - Should we must have medium recoils? (conservation of energy?) 
           - Side note: Are all the models conserving energy and momentum? (not all of them for sure) \textcolor{red}{MW: if this is detailed later, it might be worth to forward this to later. It might be also interesting to try to make a bridge to hadronisation models, mentioning that this is also not fulfilled in coalescence pictures}
           - Is there an option that we can ignore medium recoil contribution?
           - Why is medium recoil effect important? What do we learn about the QGP? (shows it is really there and we dig a hole though the QGP?)
        - Do we see evidence of medium response
           - Wide angular distribution of photon-tagged hadron spectrum, dijet missing pT shows low pT particles balance the dijet momentum imbalance
           - Enhancement of the tail part of the jet shape, soft particle enhancement in jet fragmentation function:
           - Why can't we claim victory already that we have observed medium response?
              - There are models which describe those observables without medium response (for instance, SCETg)
              - really?              
        - Do we see thermalization of medium recoils and radiated energy?
            - Are they fully thermalized? 
               - Probably not, enhancement intermediate pT particles at a few GeV
            - The failure of full thermalized description (for instance, hybrid model)
            - JEWEL - data comparison shows that the correlation between medium recoil and jet axis is too tight (no rescattering allowed)
            \textcolor{red}{I have a very naive question: how does this discussion connects to the elastic vs. radiative energy loss discussion of heavy-flavour that was there 10 years ago}

     - Lesson from it (quantitative statements, within possible, on QGP properties)
        - Transverse momentum conservation: 
           - (are we sure this is the case? Can we hide all the imbalance by forward going beam remnant or very forward going particles?)
        - If we figured out fully there is medium response and we could measure it with super high precision, what we could learn about the medium?
           - Essentially we are measuring the wake of the QGP (similar to the sound diffusion studies in atomic physics)
           - We hope to learn about the transport properties of the QGP with long wave length excitation
           - Can we connect this to the calculation of the speed of sound in Lattice? (too long shot?) \textcolor{red}{I would mention it for sure! the sound waves picture produced quite a number of papers, even if things turned out to be much more complicated. So, I think that it is important what to comment a bit how you think that a connection could be made on a more theoretical sound basis starting from measurements}



==> QGPdensity2.tex <==
\newpage
\section{Medium properties}
\label{sec:QGPDensity}

Results on soft probes, such as inclusive particle production and angular correlation analysis of low momentum hadron, have provided insights about the produced medium. Theoretical calculations, which include a high energy density, low specific shear viscosity, and thermalized medium, can describe the data from soft probes. Medium properties have been extracted from Bayesian analyses using relativistic hydrodynamics-based models, that depend on the underlying assumptions in various stages in the evolution. 

In the previous chapter, we described the medium-induced acceleration and deceleration of the hard probes. To provide additional constraints on the medium properties, we will focus on extraction with jets, heavy quarks, and quarkonia. In addition, hard probes are different from the medium particles in their transverse momentum or mass. Therefore, they have a much longer relaxation time. While soft particles lose all the memory of their initial momentum, hard probes can then be sensitive to the earlier stages of the QGP. These high momentum objects can extend the study of the created medium properties to different phase spaces because they are produced early, such as higher temperature and smaller length scales.
In the following, we will address the constraints from jets and heavy quarks on the density, stopping power (\ref{subsec:QGPdensitySopping}), and shear viscosity (\ref{subsec:QGPdensityShear}).


%In this chapter, we will discuss the extraction of the QGP characteristics from measurements of jets, heavy flavor hadrons, and quarkonia.  

%1. What is the relation between $\hat{q}$, Ds, MD, T... all those variablesin pQCD, Ads/CFT setups

%2. We compare the results (pieces of info we extract from all the obserables)

%[There is a np based calculation of qhat]

% \yj{do we have some indication or conclusion we could draw on which picture (weak or string) is prefered?} \lil{Discuss current experimental uncertainties and check what is the needed exp uncertainties from theory expectations --> Chapter 5}
%(1) Introduction of medium properties variables like qhat, g, MD, Ds, eta/s. Should this be done in Chapter 4.

%(2) It looks like the latter chapter will refer to the exp data figures in the earlier chapter, which is ok, in Chapter 5, i will put the property extraction figures or the ones which is not yet quoted before.
%(Highest precision would be the best)
%Particles and jet together.

%(3) In Chapter 5, I should focus on time integrated result and will refer to Chapter 7 for time dependence, if that's a good idea to you.
%(4) RHIC vs LHC: talk about charmonia production, connection to the diffusion. Energy gives interesting physics. RAA plot at low pT, you see a new source of j/psi from recombinationㄡ


%(5) Compare RHIC and LHC along the way. Probably a good idea to start with temperature discussion first and then go to the Density, Stopping power, diffusion discussion? 

%[h-jet LHC vs RHIC]

%Color screening, medium induced dissociation, recombination
%Different states could have different size of effects. We don't know yet at low pt for psi'.

\subsection{Density and Stopping power}
\label{subsec:QGPdensitySopping}

%[Tentative ideas]
%Talk about stopping power for cold QCD medium first?
%(1) Check with Danny if we have hybrid results on cold QCD matter
%(2) If not, then we say, based on a weak coupling method (pQCD based), we see a different in the stoppoing power (by a factor of 5-10).
%(3) from qhat to degree of freedom.
%Question: can we increase the qhat (broadening) without increasing d.o.f? 
%(4) EoS family with free parameters all indicate a speed of sound increase with medium temperature:
%https://www.bnl.gov/bes2015/files/talks/ScottPratt.pdf
%    HI Data extraction of $s/T^3$https://arxiv.org/pdf/1908.09728.pdf
%    [Drop an e-mail to Aleksi Kurkela?]
%(5) What if we don't have QGP? String models for flow and jet quenching. Are they ruled out?

%References:
%https://arxiv.org/pdf/1201.0693.pdf

%Heavy-flavour
%- elastic scattering at low/mid pt? is there evidence ? how to model 
%- hadron recoil from photons as alternative probe of this kinematic regime
%- low pt charm: is charm thermalized? point out limitations/limits based on initial state and  hadronization uncertainties 
%- bottomonium: can we use it to constrain matter properties as eta/s or alternatively the qqbar in-medium potential.

%[To be checked: Debye screening for quarkonia and heavy-flavour]

The maximum energy density occurs at the instant when the two ions overlap and collide. This density amounts to more than 12 GeV/$\rm{fm}^3$ based on the charged hadron $dN/d\eta$, $\langle p_T\rangle$ and transverse energy distribution $dE_t/d\eta$ measurements~\cite{ALICE:2010mlf,CMS:2012krf,CMS:2011aqh,ALICE:2016igk}. The energy density then decreases as a function of time as the system expands and cools down. Note that the energy density is different from the color charge density. For instance, the energy density in an electron-position annihilation can be very large, but the produced color-charged density is low. %To form a QGP after a collision, the system has to evolve towards material with a substantial color charge density at the very early stages. 
Based on measurements of total energy using inclusive particle spectra, we know that the initial energy density of the system is considerable. On the other hand, the analysis of the jet quenching imprints indicates a strongly interacting system characterized by a very high color density. However, these jet quenching analyses typically rely on several theoretical predictions and models to extract the medium properties.
%Jets and heavy quarks are colored probes that could be used to probe the color density in the medium. One needs, however, to rely on phenomenological models to extract jet transport properties and translate jet quenching information to medium properties.

\subsubsection{From jet transport coefficient to medium properties}
\label{subsec:qhatToMediumProperties}

A crucial part of the experimental programs of RHIC and the LHC is to determine the nature of the matter that is produced in ultra-relativistic heavy-ion collisions. The experimental evidences~\cite{STAR:2005gfr, PHOBOS:2004zne,PHENIX:2004vcz,BRAHMS:2004adc} that the Quark-Gluon plasma produced at both RHIC and LHC is a strongly coupled fluid may indicate that the class of weak coupling approaches may be inconsistent to retrieve information about the medium. Nonetheless, the interaction of high-momentum particles with the short-wavelength partonic excitations of the QGP will involve small QCD coupling interactions. In this quasi-particle framework, the transport coefficients introduced above within inelastic and elastic energy loss scenarios can be related to the (non-perturbative) bulk properties of the QGP, such as the shear-viscosity, $\eta$. Depending on the formalism one uses to address the determination of a jet transport coefficient, it is also possible to relate these to other bulk properties, such as energy density, $\epsilon$, or entropy, $s$. This part will focus on kinetic-transport theory as it can describe low- and high-$p_T$ particle production within the same physics dynamics. This theory provides an interpolation between free streaming (in small systems) and almost ideal fluid dynamics (in large systems). In fact, since the works in Ref.~\cite{Arnold:2002zm} with the introduction of an effective kinetic theory (EKT) to describe the transport QCD matter, EKT was applied to jet quenching phenomenology, as well as flow phenomena~\cite{Kurkela:2015qoa}. While we refer the reader to Ref.~\cite{Muller:2021wri} for details on how to derive a relation between the jet transport coefficient, $\hat{q}$ and QGP bulk properties, we present a heuristic derivation instead to illustrate how these two can be related. 

As discussed in section~\ref{sec:acceleration_energy_loss}, the jet transport coefficient is related to the differential interaction cross-section between the incoming parton and a single scattering center, $d\sigma/ dq_\perp^2$ (see eq.~\eqref{eq:sec4_qhat2}). It translates the average exchanged transverse momentum distribution between incoming parton and medium scattering center, $\left\langle k_\perp^2 \right\rangle$ per mean free path, $\lambda$. Within the framework of kinetic theory, the shear viscosity scales with the mean-free path of a constituent's particle of momentum $p$ in the medium, as well as its average thermal momentum, $\left\langle p \right\rangle$: 
\begin{equation}
    \eta \sim \frac{1}{3} \left\langle p \right\rangle \lambda \rho \, , 
\end{equation}
where $\rho$ is the density of scattering centers within the medium. Regarding the medium as a collection of quasi-particles, $\lambda = (\rho \sigma_{tr})^{-1}$, where $\sigma_{tr}$ is the total transport cross-section. When soft scattering dominates, this can be related to the differential cross-section as: 
\begin{equation}
    \sigma_{tr} = \int d\Omega \frac{d\sigma}{d\Omega} \approx \frac{4}{\hat{s}} \int d q_\perp^2 q_\perp^2 \frac{d\sigma}{dq_\perp^2} = \frac{4 \hat{q}}{\hat{s} \rho} \Rightarrow \lambda = \left(\frac{\hat{s}}{4 \hat{q}} \right)\, ,
\end{equation}
where $\sqrt{\hat{s}}$ is the centre-of-mass energy and $\Omega$ the solid angle. Taking the medium as a gas of massless thermal particles, one can use the corresponding equation of state $\left\langle p \right\rangle \approx 3T$, from which $\left\langle \hat{s} \right\rangle \approx 18 T^2$ and $s \approx 3.6 \rho$, to finally derive: 
\begin{equation}
\frac{\eta}{s} \approx 1.25 \frac{T^3}{\hat{q}} \, .
\end{equation}
This approximate relation depends on the equation of state of the medium (number of degrees of freedom), among other factors. However, our purpose here is just to illustrate that measuring transport coefficients related to the high momentum objects, such as $\hat{q}$, can elucidate the nature of the coupling strength within the medium. This relation is the reason behind all the attempts to obtain a numerical value for this phenomenological parameter. In particular, a larger value of $\hat{q}$ will imply that the medium is strongly coupled. In contrast, a smaller $\hat{q}$ could indicate the presence of a marginally weak coupling medium~\cite{Muller:2021wri}.

Despite the very different ways to deliver $\hat{q}$, it is still possible to compare its value across the different results with some care. This can be done by taking into account the particular conventions used, and that it must encode the average transverse momentum acquired by hard parton per unit length (or time) when traveling through the medium. %Even though this jet transport coefficient is not uniquely defined in all current formalisms addressing the analytical evaluation of jet quenching phenomena, it is possible to infer its value and parametric dependence by recalling that it is the parameter that denotes the transverse momentum acquired by a hard particle per length (or time) unit when traversing the soft medium bulk. 
Different approaches will naturally yield different parameterizations of $\hat{q}$. However, once this is inferred, the value of $\hat{q}$ can be compared across the different models.

The relation of $\hat{q}$ with the medium properties (like medium energy-density, $\epsilon$, entropy, $s$ or temperature) will rely on the QGP equation of state. Above, we mentioned the ideal gas scenario, but lattice results can also be used as input. Nonetheless, such choices do not hold for the entire medium evolution given the multitude of phases that the result of the collision will go through from the pre-equilibration up to the hadronic re-scattering phase. Energy losses during the pre-equilibration phase are still heavily under debate. Most works indicate that an absence of quenching during this initialization time seems to describe the high-$p_T$ flow harmonics present in less central collisions better~\cite{Noronha-Hostler:2016eow,Andres:2019eus}. On the other hand, it was suggested in~\cite{Noronha-Hostler:2016eow} that event-by-event fluctuations could be the main factor for the high-$p_T$ flow harmonics. 

As for the hadronic phase, one can consider a hadron resonance gas (HRG) description, thus using a hybrid equation of state using lattice and HRG inputs. The introduction of an evolving medium and subsequent time dependence on the jet transport coefficients also contributes to the significant theoretical uncertainties obtained on the $\hat{q}$ parameterization and when trying to retrieve an average $\hat{q}$ out of experimental results. As an example, one can look to \cite{JET:2013cls}, where five different approaches were used to retrieve the corresponding $\hat{q}$ value using high-$p_T$ single hadron measurements from both RHIC and LHC. Other similar attempts include \cite{Andres:2016iys,Xie:2019oxg,Feal:2019xfl,Xie:2020zdb} and most recent one was made by the JETSCAPE Collaboration, in \cite{JETSCAPE:2021ehl}. The models used in ~\cite{JET:2013cls} were Higher-Twist (BW and M), MARTINI, and McGill-AMY. In each of them, the $\hat{q}$ dependence on QGP parameters follows a different parameterization. In the Higher-Twist-BW, the definition of $\hat{q}$ is assumed to be proportional to the local partonic QGP density, $\rho_{QGP}$ modeled by an ideal gas at a temperature $T$,  $f$ denotes the fraction of the hadronic phase. Further considerations of a fast-evolving medium yield the dynamical parameterization on the space, $r$ and time $\tau$:
\begin{equation}
\hat{q} (\tau, r) = \left[\hat{q}_0 \frac{\rho_{QGP} (\tau, r)}{\rho_{QGP} (\tau_0, 0)} (1-f(\tau,r)) + \hat{q}_h (\tau, r) f (\tau,r) \right] \frac{p \cdot u}{p_0} \, ,
\end{equation}
where $\hat{q}_0$ denotes the transport coefficient for a parton located at the center of the QGP bulk ($r = 0$) and initial time ($\tau_0$), $p^\mu$ is the 4-velocity of the jet and $u^\mu$ the four flow velocity in the collision frame. The $\hat{q}_h$ is approximated by the meson and baryon densities, $\rho_M$ and $\rho_B$, in the HRG at a given temperature $T$:
\begin{equation}
\hat{q}_h = \frac{\hat{q}_N}{\rho_N} \left[ \frac{2}{3} \sum_M \rho_M (T) + \sum_B \rho_B(T) \right] \, ,
\end{equation}
where $\hat{q}_N$ is the jet transport coefficient from cold nuclear matter effects, extracted from DIS experiments, and $\rho_N$ the nucleon density in the center of a large nucleus. By contrast, in MARTINI, the interaction potential is derived from hard-thermal loop, where, at leading order, $\hat{q} = \hat{q} (E, T, \mu_D)$, with $E$ the energy of the incoming particle, $T$ the medium temperature and $\mu_D$ the Debye mass from the elastic potential, and an additional free parameter $C$:
\begin{equation}
    \hat{q} \approx C_R \frac{42 \zeta(3)}{\pi}\alpha_s ^2 T^3 \ln \left( \frac{2 C E T}{4 \mu_D^2} \right) \, .
\end{equation}
The other models may use different model assumptions, and we refer the reader to the original manuscripts. These are just examples to emphasize the uncertainties on obtaining a $\hat{q}$, which may involve parameterizations with additional free parameters.

%Another pressing difficulty is to account for the full parton shower evolution, which includes medium-induced interactions from softer fragments of the parton shower with the thermal medium. To overcome these obstacles, one approach is to use ad-hoc parameterizations of $\hat{q}$, involving additional free parameters. The extracted temperature and momentum dependence of the $\hat{q}$ could depend on the functional form of the parameterizations, in particular, in the extrapolation of the $\hat{q}$ results to higher temperature. In fact, the most recent attempt to withdraw jet transport coefficients from experimental data was conducted by JETSCAPE, a general multi-stage approach to in-medium jet propagation. With this setup, in \cite{JETSCAPE:2021ehl}, it was tested the outcomes from a Bayesian analysis using both RHIC and LHC results on inclusive hadron suppression, $R_{AA}$, when using MATTER + LBT models to describe the high-virtuality and low-virtuality of the parton shower development through a second-order relativistic hydrodynamic medium as provided by VISHNU2+1. The initial conditions are taken from a Monte Carlo Glauber model. Namely, the initial entropy density profile is evolved with dissipative fluid dynamics, starting at a fixed initialization time of $\tau_0 = 0.6~\rm{fm/}c$. Before the initialization time, the system is free streaming. Event-by-event fluctuations are also discarded. All parameters, but $\hat{q}$ (and its related free parameters) are fixed. Within the uncertainties, the results on $\hat{q}/T^3$ for RHIC and LHC energies agree with previous results, yielding a $\hat{q}/T^3 \sim \mathcal{O} (1-10)$, depending on the temperature and incoming particle energy. 

While these exercises help build a qualitative picture of the QGP inner workings, an accurate determination of the QGP properties is still bound by the current theoretical uncertainties to describe simultaneously perturbative and non-perturbative interactions. With the continuous progress to achieve a unified description of a coupled jet-medium evolution, more systematic studies will allow to extract, with higher accuracy, fundamental properties of the QGP using hard probes.  

%\lil{do we mention the puzzle between RHIC and LHC or do we consider it as "solved/old-fashioned"?}
%\mw{this is a general comment, als to the HF part: we end often in quite general terms that things will get better: should we indicate some directions here, shall we summarize in the end or will this become a bare enumeration that doesn't too much?}\yj{I think we can, we could discuss}
%\textbf{introduce QGP PDF.
%Initial conditions dependence
%using event-averaged hydrodynamic profiles for jet evolution 
%Limitations on possible constrains of EoS
%relation of this value to other approaches???
%relevance of event-averaged over event-by-event analysis?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figures/properties/compliationPlot_Qhat.pdf} 
\caption{A snapshot of $\hat{q}$ extracted from charged hadron spectra~\cite{JETSCAPE:2021ehl,Andres:2016iys,JET:2013cls,Xie:2019oxg,Feal:2019xfl,Xie:2020zdb} as a function of temperature. A gray area was also shown in order to cover the central values of the extracted $\hat{q}$ from different models for demonstration purpose.}
    \label{fig:CompilationQhat}
\end{figure}


\subsubsection{Input from jet measurements}

The nuclear modification factors of high transverse momentum charged particles are significantly lower than 1. This shows that the fast-moving hadrons are suppressed. Moreover, with the photon-tagged and Z-tagged jet measurements, a significant modification of the jet $p_{T}$ spectra is observed. The mean ratio of the jet and electroweak boson transverse momenta is shifted to a lower value, providing model-independent evidence that the quarks and gluons lose energy inside the medium. Since the quarks and gluons are mainly interacting with the medium through strong interaction, this shows that the color density of the produced state cannot be reproduced by a hadron gas. Nuclear modification factors of jets are also studied in AA collisions in different centrality classes. The suppression of the jet is strongest in the head-on collisions and the weakest in the peripheral events. It is not yet conclusive when the jet quenching effect has become negligible in AA collisions. On the other hand, many searches for jet quenching effects have been carried out in smaller collision systems such as XeXe and pA collisions. In XeXe collisions, the results are consistent with the expectation from theoretical models, replacing Pb ion with a smaller Xe ion. The situation in pA and dA collisions is not yet clear. While a significant flow-like signal is observed in pA collisions, there was no convincing evidence that jet quenching is observed in those smaller collision systems. Hard and soft probes are consistent with a picture of a high color density system in PbPb and gold-gold (AuAu) collisions. %It is clear that the physics picture of a high color density state in central PbPb and AuAu collisions extracted from hard and soft probes are consistent. 
However, as discussed in section~\ref{sec:smallsystem}, it is not yet conclusive whether this continues to hold in smaller and more dilute systems.
% For instance, a 60 GeV jet tagged by the photons has around 15\% of the energy transferred out of the R=0.4 cone due to the medium modification. 

As discussed in the previous section, to quantify the stopping power of the medium, the jet quenching parameter $\hat{q}$ has been extracted using the nuclear modification factors of the high transverse momentum particles. Examples of such kind of model-dependent extractions are summarized in Figure~\ref{fig:CompilationQhat}, which is currently extracted only from charged particle spectra or dihadron correlation functions. In those models, many different assumptions are used in the extraction of the $\hat{q}$:

\begin{itemize}
    \item The initial state of the heavy-ions right before the collision and its factorization with respect to final state effects
    \item The evolution of the collision bulk and the jet-medium interaction before the formation of the QGP
    \item The hydrodynamical expansion simulation of the QGP could lead to different temperature and energy density profiles as a function of time
    \item The jet quenching mechanism, start and end time of the quenching effect during the bulk evolution (energy loss during a partonic phase or also including a hadronic phase)
    \item The hadronization of the medium and hard probes
    \item The considered medium degrees of freedom (gluon gas, $N_f = 3$ quark flavors,...)
    \item The propagating particle, as gluons will lose energy with $C_A = 3$, while quarks lose energy with $C_F = 4/3$. 
\end{itemize}

% reduce the differences between the different approaches listed in~\ref{fig:CompilationQhat}, we translated, whenever possible, the considered degrees of freedom to a gas of massless particles such that:
%\begin{equation}
%    \hat{q} = 1.25 \frac{T^3}{\eta/s} \, .
%\end{equation}
Results on ~\cite{Feal:2019xfl} (X. Feal at al) report $\hat{q}/T^3$ for a gluon propagating through a medium while \cite{JET:2013cls} (JET Collaboration) refer to a quark. These are then the limiting cases while the remaining models present an average $\hat{q}/T^3$ that will contain a mixture of the two contributions. To illustrate this change, we re-scaled the results from~\cite{Feal:2019xfl} by $C_F/C_A = 4/9 \simeq 0.45$ to include the equivalent for the quark as well. The results for the extracted $\hat{q}/T^3$ of quark-initiated jets do not agree between the different approaches as the remaining ingredients used in each model differ substantially. The assumptions regarding the initialization time of the QGP usually range from $\tau_0 = 0.6$~fm/$c$ up to $\tau_0 = 1.0$~fm/$c$. All but~\cite{Andres:2016iys} (C. Andrés et al.) neglect energy loss effects before this initialization time. The effect of changing this assumption solely is illustrated  in this reference. In Fig.~\ref{fig:CompilationQhat}, we decided to include only the free-streaming option with $\tau_0 = 0.6$~fm/$c$, but variations of $20\%$ in the extracted $\hat{q}/T^3$ are also to be expected, depending on the considered medium temperature. As for the model adopted for the medium, in \cite{Feal:2019xfl, JET:2013cls}, it is assumed a Stefan-Boltzmann gas of quarks and gluons, while in \cite{Andres:2016iys,JETSCAPE:2021ehl,Xie:2019oxg} a hydrodynamical model is employed instead. In this case, the initial conditions must be specified. In~\cite{Andres:2016iys}, it was explicitly considered in their calculations two examples: a factorized Kharzeev-Levin-Nardi (KLN) model~\cite{Drescher:2006pi} and the Hirano model~\cite{Hirano:2001eu}. The corresponding results, to illustrate the sensitivity of $\hat{q}$ to these effects, are also shown in Figure~\ref{fig:CompilationQhat}. The jet-medium interaction model is also different among all considered approaches. For instance, in~\cite{JETSCAPE:2021ehl} (Jetscape), the extracted $\hat{q}$ and corresponding uncertainties are shown when using MATTER to describe energy loss processes (pink shaded region) or a Linear Boltzmann Transport Model (LBT, light orange shaded region). Most of the data sets used in these approaches are constrained to single charged particles to avoid reconstruction biases. However, to overcome this effect, in~\cite{Xie:2019oxg} (M. Xie et al.), a global $\chi^2$ analysis on the nuclear modification factor for single and double hadron production at RHIC and LHC energies is adopted. While at RHIC energies, the fitting results from using one or both data sets are consistent, there are differences in the used data set at LHC energies. In Fig.~\ref{fig:CompilationQhat}, only the combined result is shown, but the extracted $\hat{q}$ would be larger for double hadron production given that the observed suppression in this observable is also proportionally larger. 

While an accurate determination of the extracted $\hat{q}/T^3$ is not yet possible (the central value can vary by a factor of up to 6) the temperature dependence of this parameter can already be withdrawn. First attempts were indicating an additional dependence with $\sqrt{s}$ as, for the same medium temperature, results from RHIC and LHC data were not consistent. With the most recent efforts to include more accurate descriptions of jet-medium interaction, it is now clear that $\hat{q}/T^3$ does not depend on the collision system, but rather only on the medium characteristics. With the continuous progress on the analytical description of jet quenching phenomena, we expect the novel qualitative features brought by the hard sector to contribute to the narrowing of the current uncertainties. 

In addition, future use of additional data sets to extract $\hat{q}$ will also help to bring a more unified description. Inclusive charged hadron spectra focus only on the leading fragment of the event. A global analysis with other configurations has already proved challenging~\cite{Xie:2019oxg} given the current theoretical uncertainties on how to describe a multi-partonic system developing through an evolving medium. It was recently shown that jet substructure observables such as jet splitting functions, an almost completely orthogonal measurement to jet and hadron spectra, are sensitive to the magnitude of $\hat{q}$~\cite{Mehtar-Tani:2016aco,Chien:2016led,Milhano:2017nzm,Chang:2017gkt}. Determination of jet transport coefficients from jet spectra, jet substructure, or both could be an important test in the future and complementary to the studies that have been done with inclusive hadron spectra and dihadron correlation functions.

In the angular correlation measurements of two hard observables at large angular differences, such as photon-jet~\cite{Chatrchyan:2012gt,CMS:2017ehl,ATLAS:2018dgb}, dijet~\cite{ATLAS:2010isq,CMS:2011iwn}, Z-jet~\cite{CMS:2017eqd} and hadron-jet~\cite{ALICE:2015mdb,STAR:2017hhs} correlation, one hopes to learn about the medium structure through Rutherford-experiment-like measurements. Currently, all such measurements in AA collisions are consistent with pp references, and there is no indication of back-scattering in the experimental data. This shows that the produced medium is very smooth using the currently accessible high momentum particles, consistent with the physics pictures used in the soft sector modeling. More detailed studies with high statistics data at higher and higher particle transverse momentum could help resolve the QGP structure at shorter scales~\cite{Busza:2018rrf}.

%QGP density extracted from jets / high pT particles. We learned from charged particles RAA that the high transverse momentum particles are suppressed. We also learned from jet RAA that a clustering algorithm can not recover all the jet energy. Finally, photons are not modified significantly and the modification of their pT and rapidity spectra are related to the initial stage effects. Photon-tagged jets spectra: unambiguous measurements which shows jet clustering can not capture as much initial parton energy as that in pp collisions. This shows the color density and stopping power is very high (rough estimation). 

%To determinate the stopping power quantitatively, currently, the qhats are extracted from charged particles only. (Jet collaboration, jetscape, etc). 

%\begin{figure}
%    \centering
%    \includegraphics[width=0.6\textwidth]{figures/properties/jetscapeQhat.JPG} 
%\caption{Qhat}
%    \label{fig:jetscape}
%\end{figure}


%Charged particle v2: delay of the jet quenching vs. time. Recently extended to jet substructure.  Model independent eloss extraction (xin-nian paper)

%Figure: ALICE / CMS / ATLAS charged particle RAA, jet RAA
%Figure: CMS/ALICE/STAR jet splitting function

\subsubsection{Input from Heavy flavor hadrons}

In chapter~\ref{sec:acceleration}, we reviewed a collection of precise measurements from the LHC experiments and the RHIC upgrades that have brought heavy-flavor hadron measurements to a new level of precision. This was accomplished by allowing to reconstruction of weak decays with lifetimes between $50-500$ $\mu$m in exclusive decay chains of specific hadrons experimentally via modern silicon vertex detectors. The measurements in the heavy flavor are well in line with the expectations from a strongly coupled QGP. Despite the expected longer relaxation time, there is a strong nuclear modification of production yields and participation in the collective motion visible via the large elliptic flow and triangular flow. A large number of models can describe the open-heavy flavor data implementing different types of transport equations. However, the model constructions and inputs vary significantly and need to be brought on a common assumption as outlined in Ref.~\cite{Rapp:2018qla} to allow for more quantitative conclusions. Even full thermalization is a scenario that is not excluded by experimental data~\cite{Andronic:2021erx}. Furthermore, to scope with the complex problem, today's modeling is making a rather schematic idealization of the initial state, mostly semi-classical propagation descriptions in the QGP and a hadronization prescription. However, it is dealing, nevertheless, with a large assumption and parameter space. This picture has served us well to identify qualitative interpretations with quite different approaches. With increasing experimental precision and the desire to extract matter properties, the assumption of factorization in the description of the initial state, the role of pre-equilibrium dynamics and escape mechanism, the approximations required to justify a specific transport equation, suited as a starting point, need to be tested more systematically with theory and experiment and possibly revised.  Independent of conceptual model limitations and ambiguities, at the current stage of understanding and within all current 'frameworks', it is mandatory to improve the knowledge on the initial state and hadronization. The associated uncertainties largely dominate standard observables like nuclear modification factor and elliptic flow, as we illustrate in chapter~\ref{sec:initial} and~\ref{sec:hadronization}.  The latter inputs on the experimental side will soon improve significantly with increasing statistics from the experiments. 

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figures/properties/Ds_Review2021.pdf} 
\caption{A compilation of the charm-quark spatial diffusion coefficient, $2\pi T{\cal
D}_s$, presented over a wide range of reduced temperature $T/T_{\rm C}$. Below the pseudo-critial temperature $T_{\rm C}$, the results for $D$ meson diffusion using effective hadronic interactions~\cite{He:2011yi,Tolos:2013kva} are shown. Above $T_{\rm C}$, results from quenched lattice QCD \cite{Banerjee:2011ra,Ding:2012sp,Kaczmarek:2014jga,Brambilla:2020siz,Ding:2021ise,Francis:2015daa,Altenkort:2020fgs} are shown as the data points with vertical error bars and compared to anti--de Sitter/conformal field theory (AdS/CFT)-based calculations~\cite{Horowitz:2015dta}. In addition, various model calculations based on LO pQCD~\cite{Moore:2004tg,vanHees:2004gq}, quasi-particle model (QPM) calculations utilizing Boltzmann-based extractions (BM) or Langevin-based extractions (LV)~\cite{Das:2015ana}, a dynamical QPM model in Parton-Hadron-String Dynamics (PHSD)~\cite{Song:2015sfa}, $T$-matrix based calculations with free energy ($F$) or internal energy ($U$) as potential~\cite{Riek:2010fk} and the Monte Carlo at Heavy Quarks (MC@sHQ) perturbative approach with running coupling~\cite{Andronic:2015wma} are also shown. Finally, a data-driven extraction based on a Bayesian analysis is shown as a red band, presenting the 90\% confidence-interval in the Duke hydro/transport model. }
    \label{fig:CompilationDs}
\end{figure}

Heavy-flavor observables can be used as a tool to constrain the heavy-quark diffusion coefficient. As in the light-flavor sector, one needs to consider a specific model ansatz and fix the input assumptions. Bayesian fits have demonstrated the coefficient sensitivity to the experimental results in several approaches. As an example, the attempt to extract the spatial quark diffusion coefficient $D_{s}$ of heavy quark, similarly to the extraction of matter properties in the soft sector~\cite{Xu:2017obm}. A compilation of the results from the theoretical calculations~\cite{Rapp:2018qla,Cao:2018ews} together with the mentioned data-constrained extraction~\cite{Xu:2017obm} are shown in Figure~\ref{fig:CompilationDs}.

Measurement-driven improvements of our input knowledge on the initial state and hadronization in different collision systems will hopefully guide phenomenology to reduce the spread of parameter space. In view of heavy-flavor transport, bottom observables will allow becoming more quantitative at the interface between model and theory thanks to the larger quark mass.   


\subsubsection{Input from Quarkonia}

The investigation of quarkonia in heavy-ion collisions at RHIC and at the LHC brings two qualitatively new insights: the sizeable regeneration of J/$\psi$~\cite{ALICE:2012jsl,ALICE:2013osk,ALICE:2015nvt,ALICE:2015jrl,ALICE:2016flj,ALICE:2017quq,ALICE:2018bdo,ALICE:2019lga} and the sequential suppression of the $\Upsilon$-states~\cite{CMS:2011all,CMS:2012bms,CMS:2012gvv,STAR:2013kwk,PHENIX:2014tbe,ALICE:2014wnc,CMS:2016rpc,STAR:2016pof,CMS:2017ycw,CMS:2018zza,ALICE:2019pox,ATLAS-CONF-2019-054,ALICE:2020wwx}. Both observations are interpreted as most directly possible signatures of deconfinement. The observation of their modification and its interpretation connects them with open-heavy flavor observables. First, there is a connection via the allowed 'coupling' of the single heavy quark and the quarkonium via regeneration. In addition, on the theoretical ground, when the QGP 'resolves' the quarkonium constituents, it is possible to link between the interactions of heavy quarkonium with those of single heavy-quarks.  %also present between simple  %via the appearance of the heavy-quark diffusion in the description of dynamical quarkonium modeling.
We just start to go beyond qualitative findings. The degree and moment of regeneration cannot be decided for charmonium states based on current experimental results. Here, the constraints on the initial condition of total $c\bar{c}$ and more precise measurements of a larger number of quarkonium states should bring progress.  For bottomonium, the sensitivity to the heavy-quark potential, and hence the Debye mass as well as to heavy quark diffusion coefficient, have been demonstrated in the literature. However, here, the classes of models used to describe the data are very broad. There is the need for constraints on initial densities and precise feed-down information to exploit the observed sensitivity beyond the scope of model-dependent statements.  


%\mw{ The measurement of heavy flavor hadrons allow to tag massive partons. The large mass of the beauty and charm quark allows to  vary the relative size of elastic and radiative energy loss.  In particular at low transverse momentum, we can access the heavy-quark diffusion coefficient. comment on RAA, v2 and on consistency with theory, see older emmi report. explain uncertainties independent of interaction modelling: initial state and hadronization (other chapters)}
%Discuss the dead cone effect. Show ALICE and CMS compilation plots.  High $p_T$ quarkonia: jet quenching. \mw{gluon tagging?} Quarkonia $v_2$ into the insights about if charm diffusion. 

%\mw{Quarkonia: 
%The experimental observation of larger nuclear modification factor of J/$\psi$ at the LHC vs RHIC, rapidity dependence. signature of deconfined medium. charm quarks approaching thermalization. Bound state as multi-scale test of strongly coupled QGP picture.    
%Upsilon:  describe inputs: bulk, interactions between quark-pair and hadronization, initial state,  assuming model sensitivity to medium properties as eta/s (consistent within model) , quark-antiquark interaction modelling: choose theory to probe. Systematic improvement of quark-pair interaction via LQCD and effective field theory. Importance of non-static problem, quantum effects to be taken into account.    put forward for heavy-flavour: initial state and hadronization as main uncertainties, quarkonium included. 
%}

%\begin{figure}
%    \centering
%    \includegraphics[width=1\textwidth]{} 
%\caption{[Figures: ALICE + RHIC J/psi}
%    \label{fig:splittingFunction}
%\end{figure}

%\begin{itemize}
%    \item Density of the QGP
%    \begin{itemize}
%        \item QGP density and qhat from high pt objects (jets, particles)
%        \item  A short reminder of Density of the QGP from particle dN/deta, <pT> and dEt/deta. What %are the underlying assumptions?
%        \item Why is QGP density and qhat important and how they can be related
%        \item What is the current status of the qhat extraction (largely based on particles %only(!))?
%        \begin{itemize}
%            \item Why do we still have a sizable uncertainty? (Underlying mechanism). 
%            \item Why is the extraction of qhat from particles not enough and can't we just work on %particles?
%            \item What would be the qhat extracted from jets and jet substructre based observables? %Are they consistent with the extracted values from charged particles?
%            \begin{itemize}
%                \item What can we say about qhat from jet RAA?
%                \item What is the expectation on the modification of dijet or photon-jet angular %correlation?
%                \item qhat extraction from Zg
%            \end{itemize}
%            \item Suppose we know very well the qhat, what do we learn?
%        \end{itemize}
%        \item eta/s from quarkonia (changes the lifetime of the medium)
%        \item Short reminder / reference of the eta/s extraction from flow
%        \item Different eta/s changes the way QGP evolve (lifetime, density evolution etc) in hydro %model. Leads to different suppression pattern of quarkonia
%    \end{itemize}
%    \item Temperature of the QGP
%    \begin{itemize}
%        \item short reminder of thermal photon extraction
%        \item Quarkonia are sensitive to temperature. What do we know about the temperature of QGP %and consistency between different measurements
%    \end{itemize}
%    \item diffusion coefficient from heavy-quarks (also connect to eta/s in some way.)
%    \begin{itemize}
%    \item Why is diffusion coefficient important?
%    \item Lattice predictions, pQCD based predictions for charm and beauty quark diffusion
%    \item Extraction from D meson v2 and RAA. Why can't we claim victory already?
%    \item Why do we want to study beauty quarks? (heavier) 
%    \item Can we relate Ds and eta/s? Do we see an overall consistent picture or not?
%    \item Why is it important to further improve the diffusion coefficient measurement with future %data?
%    \end{itemize}
%\end{itemize}

%\subsection{Temperature of the medium}

%Extraction of temperature was performed with thermal photons (refer to review). Inclusive Quarkonia $R_{AA}$ tell us about the temperature of the medium. Measurement from RHIC vs LHC: higher temperature at the LHC compared to RHIC. 



\subsection{Specific Shear Viscosity}
\label{subsec:QGPdensityShear}

The ratio of shear viscosity and entropy, often referred to as specific shear viscosity, is a dimensionless quantity and an important transport coefficient of matter. It has been studied extensively in various systems. Figure~\ref{fig:CompilationShearViscosity} summarizes the current status of the extracted specific shear viscosity ($\eta/s$). The $\eta/s$ extracted from a Bayesian analysis (labeled as "QGP (Soft Probe)") on low transverse momentum spectra and hydrodynamics flow is compared to other media such as water, helium, a calculation of fermionic quantum liquids (Fermi gas)~\cite{Enss:2010qh}, and a calculation based on a string theory method for a large class of strongly interacting quantum field theories whose dual description involves black holes in anti-de Sitter space (AdS/CFT)~\cite{Kovtun:2004de}. The results from Bayesian analysis are close to calculations from AdS/CFT and smaller than those from other media, at around a factor of 10-20 smaller than water and helium and a factor of around 5 smaller than the calculation of Fermi gases. This shows that the QGP is very strongly interacting and the closest medium to ideal fluids.

It is of great interest to check this conclusion using hard probes. In order to compare the transport properties extracted from jet quenching and from heavy quark diffusion in the medium, we performed model-dependent translations. As an example, we chose to use
\begin{eqnarray}
\frac{\eta}{s}=1.25 \frac{T^{3}}{\hat{q}}
\end{eqnarray}
as discussed in Sec.~\ref{subsec:qhatToMediumProperties}. This relation holds under the assumption of multiple soft emissions and gas of massless particles. Other equation of states would yield a different result, but this allows us to have an overall qualitative picture of the landscape of the $eta/s$ phase space. % and we therefore put this as different but we use this to illustrate in the multiple soft limit, from jet quenching via various models extracted parameter $\hat{q}$  is related to $\eta/s$ by the following relation:

The results are close to the extracted values from the hydrodynamic flow. However, the spread of the extracted $\hat{q}$ values between various theoretical models is still substantial due to the underlying jet quenching mechanisms, initial state, and hydrodynamics models used in the theoretical calculations. Note that the extended reach shown in the jet quenching result to large temperature comes from a model-dependent parameterization, dominated by the data-driven extractions from theoretical models~\cite{JETSCAPE:2021ehl,Andres:2016iys}.

Nonetheless, we can still check if, within the large uncertainties, there is consistency between heavy quark and the picture seen by the soft probes. The heavy quark spatial diffusion coefficient $D_s$ values extracted from a Bayesian analysis~\cite{Xu:2017obm} is also translated to $\eta/s$ using the following relation:
\begin{eqnarray}
\frac{\eta}{s}=\frac{Ds(2\pi T)}{ 4\pi k} \, ,
\end{eqnarray}
where the scale factor $k$ ranges between 1 and 2.5 due to the difference between pQCD and AdS/CFT based calculations. The results from soft probes, jet quenching and heavy flavor are consistent with each other, despite the large uncertainties associated with theory and experimental accuracy.

\subsection{Outlook}
\label{subsec:Outlook}

Even though jets have more solid inputs from theory than the calculations of heavy flavor and quarkonia, the lack of a complete jet-hydro coupled description within a theoretical framework blurs a quantitative extraction of the QGP transport properties. On the other hand, it is still possible to extract the big picture from the current state-of-art jet quenching models. The extracted transport properties are consistent with that from soft probes.

Heavy quark transport coefficient extracted from heavy flavor hadrons could benefit from the extensive heavy-ion data to be collected in Run 3+4 at the LHC and with sPHENIX at RHIC. Further theoretical developments may provide a better understanding of charm and beauty hadronization. These will be discussed in Chapter~\ref{sec:hadronization}.

The different modeling of the early stages of the heavy-ion collisions and the time-dependent evolution of the QGP contributed significantly to the theoretical uncertainties associated with heavy flavor and jet calculations. With hard probes, it is possible to extract useful information in a time-differential way to be sensitive to different parts of the medium evolution. Those ideas and future opportunities will be discussed in Chapters~\ref{sec:timescale} and~\ref{sec:outlook}.

%Viscosity from soft particles. Translation of Ds to eta/s from AdS/CFT (hf review discussion). The results from soft particles and heavy flavor mesons are consistent with each other, however, the theoretical (model dependence, translation from Ds to eta/s) and experimental (statistics and systematics) uncertainty from Ds is still very big. Comment on the future improvement at the end. 

%Figure: viscosity results from Duke group and a simple tranlation from Ds to eta/s


\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figures/properties/compliationPlot.pdf} 
\caption{Compilation of the specific shear viscosity as a function of temperature of the medium. To compare the properties various media close to phase transition temperature, the temperature is normalized by the (pseudo-~)~critical temperature of the medium. A model dependent translation of jet quenching parameter $\hat{q}$ and heavy quark diffusion coefficient $D_s$ to specific shear viscosity is performed and the results shown as QGP (Jet quenching $\hat{q}$) and QGP (Heavy Flavor $D_{s}$) in the figure. }
    \label{fig:CompilationShearViscosity}
\end{figure}

\clearpage

%\begin{figure}
%    \centering
%    \includegraphics[width=1\textwidth]{figures/properties/Upsilon.png} 
%\caption{Qhat}
%    \label{fig:UpsilongShearViscosity}
%\end{figure}


%\subsection{Thermalization and medium response}
%\label{subsec:thermalization}


%What is the motivation to study the thermalization of hard probes? 

%Hard probes could also be used to provide a reference axis. There are associated production of softer particles which could be used to study the thermalization of the soft part as well. 


%With hard probes: we look at the thermalization process

%Point out that future measurements with identified spectra associated with jets would be very useful (with ALICE, CMS MTD etc)

%\begin{itemize}
%    \item With hard probes: we look at the thermalization process
%    \item Can we say more beyond the statement above? for instance, what can we learn about the initial stages of the QGP if we learned how the (semi-)hard probes thermalize?
%    \begin{itemize}
%        \item connection to kinetic theory and hydrodynamization
%    \end{itemize}
%\end{itemize}
    

%\subsubsection{Thermalization of jets}

%Softening of the jet, modification of the jet constituent and jet substructure as indication of termalization. Experimental data shows that the soft component is thermalized first while the hard component is never fully thermalized. 

%[Look at the jet tagged particle spectrum from CMS and ATLAS, Z-tagged particle spectrum from CMS/ATLAS to see if we could conclude something.]


%\subsubsection{thermalization of heavy quarks}

%Elliptic flow and RAA of heavy quarks. Jet-D correlation. The hard part of the jet is not thermalized while the soft part is modified significantly.

%Figure v2 of heavy quarks, jet fragmentation and jet shape

%\begin{itemize}
%    \item What is thermalized first? (Soft component)
%    \item What is never thermalized? (hard part of the jet)
%    \item What is the connection to charm (or beauty) thermalization? 
%\end{itemize}

%\subsection{Medium response to fast moving quarks}

%To measure the transport properties, the most intuitive way is to disturb the medium and observe how the system evolves. Through missing transverse momentum, jet-hadron, photon-hadron and Z-hadron correlation measurements, the results show a strong indication of a medium response to the fast moving parton in the form of associated low transverse momentum particle production from low to large angle (at least up to $\Delta R \sim 2$) with respect to the hard probe axis. Those results are consistent with a wide range of interpretations, from basic medium recoils, wake,  to reheating of the QGP. Those results are consistent with interpretation of the flow signal in the soft sector. However, the detailed information such as particle compositions and lowest momentum component of the associated hadrons are not yet available experimentally.



%Based on the conservation of energy, there must be medium recoils and medium response. First explain medium recoil, medium response. 

%Dijet asymmetry and Jet RAA: show energy flow out of jet cone. Jet missing pT: very far away from the jet. Finally jet shape: quantify the amount of modification. 
%Issue: many jet quenching models could explain the same observable satisfactorily. They contain different amount of jet induced medium excitation. 

%Medium response/recoil (long wave-length behaviour)
%\begin{itemize}
%    \item Should we must have medium recoils? (conservation of energy?) 
%    \item Side note: Are all the models conserving energy and momentum? (not all of them for sure)
%    \item Is there an option that we can ignore medium recoil contribution?
%    \item Why is medium recoil effect important? What do we learn about the QGP? (shows it is really %there and we dig a hole though the QGP?)
%    \item Do we see evidence of medium response:
%    \begin{itemize}
%%pT particles balance the dijet momentum imbalance
 %       \item Enhancement of the tail part of the jet shape, soft particle enhancement in jet %fragmentation function:
%        \item Why can't we claim victory already that we have observed medium response?
%        \item There are models which describe those observables without medium response (for %instance, SCETg) - really?
%    \end{itemize}
%    \item Do we see thermalization of medium recoils and radiated energy? Are they fully %thermalized? Probably not, enhancement intermediate pT particles at a few GeV
%    \begin{itemize}
%        \item The failure of full thermalized description (for instance, hybrid model)
%        \item JEWEL - data comparison shows that the correlation between medium recoil and jet axis %is too tight (no rescattering allowed)
%    \end{itemize}
%\end{itemize}

%\subsection{Flavor content of the medium}
%Parton fragmentation (string fragmentation) was especially successful. Coalescence mechanism could contribute. 
%Low pT j/psi at LHC (ALICE) and RHIC.

%With it, we could study the medium flavor content by an external probe. 

%\subsection{Remaining issues on the current interpretation}

%Lesson from it (quantitative statements, within possible, on QGP properties). Transverse momentum conservation: checked with mpt. Medium response interpretation vs radiative energy loss for out of cone soft particle enhancement. Hadronization effects of the charm and beauty and total charm / beauty cros-section [refs]. 




%\begin{itemize}
%    \item Transverse momentum conservation:  (are we sure this is the case? Can we hide all the imbalance by forward going beam remnant or very forward going particles?) dijet missing pT
%    \item If we figured out fully there is medium response and we could measure it with super high precision, what we could learn about the medium?
%    \begin{itemize}
%        \item Essentially we are measuring the wake of the QGP (similar to the sound diffusion studies in atomic physics)
%        \item We hope to learn about the transport properties of the QGP with long wave length excitation
%        \item Can we connect this to the calculation of the speed of sound in Lattice? (too long shot?)
%    \end{itemize}
%\end{itemize}


==> accelerationdeceleration.tex <==

\section{Acceleration and deceleration of the probes: the short wave-length behaviour}

\begin{itemize}
    \item Introduce basic concept of vacuum dynamics 
    \textcolor{red}{MW: term vacuum dynamics: you mean 'dynamics' of hard pQCD process? hard partonic scattering, parton splittings, shower, hadronisation?}
    \yj{Probably we should also refer to a vacuum reviews.}
    \item QGP presence will lead to medium-induced modifications that will
    \begin{itemize}
        \item degrade energy of particles
        \item deflect particles direction (link to next section)
        \item modify hadro-production (link to IS)
        \item (bullets below)
        \item theoretical link between energy loss and deflection (depends on the number of emitted particles)
    \end{itemize}
    \yj{There are some links between degrade and deflect. Also for some of the observables, there are nature decorrelations like ISR effects (suitable for the vacuum dynamics part?)}
    \item Current methodology: theoretical modeling, comparison with data and withdraw of QGP properties (how fast particles thermalise in QGP) or put some limits to it 
    \item Strong limitation: QGP is a fast evolving medium but current knowledge requires input from Soft sector (link to future outlook to "measure" QGP evolution with Hard Probes).
\end{itemize}
\textcolor{red}{MW: the 'theoretical modeling' needs to be made clear in contrast to theory}
\textcolor{red}{MW: I agree, this looks good as structure.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model independent extraction of acceleration and deceleration}

\begin{itemize}
    \item List of main observations of energy loss and brief discussion on their results
    \begin{itemize}
        \item jets (R evolution, photon jet, RAA,...)
        \item Light and Heavy-Flavour (RAA, flow,...)
        \item Quarkonia (ccbar, upsilon,...)
    \end{itemize}
    \begin{itemize}
        \item Focus first on effects present across all observables
        \item Consistency between jets, ligth and HF 
        \item Links to next section
        \begin{itemize}
            \item Signatures of thermalization
            \item HF diffusion
            \item Presence of recombination, coalescence,...
        \end{itemize}
    \end{itemize}
    \item Discussion on interpretation limitations:
    \begin{itemize}
        \item Quarkonia production: from pp to PbPb
        \item Future QGP evolution measurement (quarkonia and jets: link to 7)
        \item Factorization between IS/FSR/Hadronization
    \end{itemize}
\end{itemize}
\textcolor{red}{MW: this looks good to me. For the last point, i am wondering whether this is specific to Quarkoniua production or generically rather hadronisation description (which is particulary problematic for quarkonium)}

\yj{Could be interesting to first point out that if we have seen acceleration and deceleration based on experimental observables}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Energy loss in final state effects}

\begin{itemize}
    \item Brief discussion on energy loss models
    \begin{itemize}
        \item basic assumptions, basic underlying theory (no specific model details), elastic and inelastic energy loss,...
        \item Factorization between soft and hard scales
        \item Monte Carlo modelling (and basic assumptions)
    \end{itemize}
    \item qhat parameters from exp (light and heavy) - first and latest results on JETSCAPE - particle RAA
        \begin{itemize}
            \item RHIC vs LHC qhat puzzle solved
        \end{itemize}
    \item QCD splittings - Lund planes, jet substructure
    \item Flavour dependence on energy loss and particle - jet comparison
    \item Outlook: 
    \begin{itemize}
        \item Lessons learned
        \item Interplay between different probes (discussion/ideas on "what else can we do?")
        \item Unified description of soft and HP (full jet, theory and MC)
        \item Data-theory comparison
    \end{itemize}
\end{itemize}
(Conclusion on gluon density and color charge density to the next section?)

\textcolor{red}{MW: I am wondering if there is something relevant for qhat outside JETSCAPE}
\textcolor{red}{MW: was the RHIC-LHC qhat puzzle important to refer to it here?}
\textcolor{red}{MW: I was wondering whether there should be a discussion of a strong vs weak coupling picture should appear somewhere (even if Ads/CFT is not discussed much any more) }
    \yj{ I believe the hybrid model is still on the market. Also another AdS drag based RAA calculations on the heavy flavor RAA}
\textcolor{red}{MW: yes, about the density, I would put it rather in the next session}

\yj{wrap the discussion around debye mass in chapter 5?}

